The facts on quantum self-dual Einstein gravity and self-dual Yang-Mills theory

Self-dual Einstein gravity is a one-loop exact, UV and IR finite, diffeomorphism invariant, non-unitary theory of quantum gravity in four dimensions. The only generically non-zero amplitudes are the one-loop-all-plus amplitudes, and they are equal to those of pure Einstein gravity. In these notes we review SDG and SDYM pedagogically. We walk the reader through key calculations, fill in some gaps in the literature, and point out directions for future research. Topics include: derivation of the self-dual actions from the full Einstein gravity/YM actions in lightcone gauge, decoupling of ghosts, Berends-Giele currents, vanishing of tree-level-one-minus amplitudes, celestial $\Lw$ symmetry, perturbiners, double-off-shell current calculation of one-loop-all-plus SDYM and SDG amplitudes, dimension shifting, unitarity cuts, the BDPR gravity formula, one-loop color ordering, perturbative dilatation symmetry of SDG, and the covariant formulations of the self-dual theories as well as their their gauge fixing. We also review some selected results from the celestial holography program.

==> jdef.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,180); %set diagram left start at 0, and has height of 180

%Straight Lines [id:da6469664806272312] 
\draw    (202.51,69.85) -- (208.08,81.43) ;
\draw [shift={(206.43,77.99)}, rotate = 244.3] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Shape: Ellipse [id:dp14035507834742977] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][fill={rgb, 255:red, 221; green, 221; blue, 221 }  ,fill opacity=1 ] (203.44,89.24) .. controls (203.44,83.08) and (212.18,78.09) .. (222.95,78.09) .. controls (233.73,78.09) and (242.46,83.08) .. (242.46,89.24) .. controls (242.46,95.4) and (233.73,100.39) .. (222.95,100.39) .. controls (212.18,100.39) and (203.44,95.4) .. (203.44,89.24) -- cycle ;
%Straight Lines [id:da26227883176678446] 
\draw    (242.33,67.89) -- (237.07,81.43) ;
\draw [shift={(238.76,77.09)}, rotate = 291.22] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da9699269105909194] 
\draw    (213.66,64.65) -- (216.63,79.2) ;
\draw [shift={(215.67,74.47)}, rotate = 258.46] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da13890834665421337] 
\draw    (222.95,100.39) -- (222.95,113.89) ;
\draw [shift={(222.95,103.04)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da6435401600193765] 
\draw    (272.47,109.91) -- (247.86,109.91) ;
\draw [shift={(244.86,109.91)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.04,-3.86) -- (0,0) -- (8.04,3.86) -- (5.34,0) -- cycle    ;

% Text Node
\draw (185.45,90.33) node [anchor=east] [inner sep=0.75pt]    {$\mathcal{J}( 1,\dotsc ,n) =$};
% Text Node
\draw (197.25,69.55) node [anchor=south] [inner sep=0.75pt]  [font=\footnotesize]  {$1^{+}$};
% Text Node
\draw (247.95,65) node [anchor=south] [inner sep=0.75pt]  [font=\footnotesize]  {$n^{+}$};
% Text Node
\draw (213.66,63.05) node [anchor=south] [inner sep=0.75pt]  [font=\footnotesize]  {$2^{+}$};
% Text Node
\draw (229.3,56.63) node    {$...$};
% Text Node
\draw (222.95,117.29) node [anchor=north] [inner sep=0.75pt]  [font=\footnotesize]  {$m^{-}$};
% Text Node
\draw (276.47,100.58) node [anchor=west] [inner sep=0.75pt]  [font=\scriptsize] [align=left] {(off shell leg, do not\textcolor[rgb]{1,1,1}{..}};
% Text Node
\draw (277.14,113.24) node [anchor=west] [inner sep=0.75pt]  [font=\scriptsize] [align=left] {amputate propagator\textcolor[rgb]{1,1,1}{....}};
% Text Node
\draw (277.14,125.24) node [anchor=west] [inner sep=0.75pt]  [font=\scriptsize] [align=left] {or include polarization)};


\end{tikzpicture}

